CrossLiDAR: Controllable Multi-Sensor LiDAR Sequence Generation

High-fidelity LiDAR simulation remains a bottleneck for scalable development and validation of autonomous systems. Existing generators can synthesize realistic scans, but they are typically constrained to a single sensor configuration, offer limited control over structure and geometry, and drift in long-horizon 4D generation. We present CrossLiDAR, a unified transformer-based framework capable of generating controllable and spatio-temporally consistent multi-sensor LiDAR sequences. Our approach leverages a rectified flow objective with a Multi-Modal Diffusion Transformer (MM-DiT) backbone, within a compact latent space of range images. To support multiple LiDAR sensors, an Inter-sensor Module enables interaction across sensors, while a ControlNet-style branch provides structural conditioning (e.g., BEV priors or 3D bounding boxes). For modeling the temporal consistency, CrossLiDAR generates short $N$-frame sequences and extends them autoregressively to improve long-horizon coherence. Our model significantly outperforms state-of-the-art baselines, achieving an average improvement of 29.56\% in JSD and 15.36\% in MMD evaluated on nuScenes and the Waymo Dataset. CrossLiDAR bridges the gap to modern autonomous-driving simulation by enabling calibration-consistent multi-sensor LiDAR rollouts over long horizons for controllable, scenario-based testing.

==> assets/tables/competitors_khanh.tex <==
\begin{table}[H]
\begin{center}
\caption{\textbf{Existing methods} for LiDAR generation. \textbf{Settings}: \emph{SS}: Single LiDAR sensor, \emph{MS}: Multi- LiDAR sensor, \emph{MV}: Multi- Camera, \emph{MM}: Multi- modality. \textbf{Datasets}: \emph{K}: KITTI-360\cite{liao2022kitti}, \emph{N}: nuScenes\cite{caesar2020nuscenes}, \emph{W}: Waymo\cite{sun2020scalability}.}
\begin{small}
\small
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccc}
\toprule
 & Venue & Frames & Setting & Condition & Dataset & Code & Checkpoint\\
\cmidrule{1-8}
LiDARGen\cite{li2022pcgen} & ECCV 22 & single & SS & -,- & K & \href{}{Yes} & K \\
LiDAR Diffusion\cite{ran2024towards} & CVPR 24 & single & SS & image,semantic map & K & \href{https://github.com/hancyran/LiDAR-Diffusion}{Yes} & K \\
RangeLDM\cite{hu2024rangeldm} & ECCV 24 & single & SS & inpaint,downsample & K,N & \href{https://github.com/WoodwindHu/RangeLDM}{Yes} & K,N\\
R2DM\cite{nakashima2024lidar} & ICRA 24 & single & SS &  &  & \href{https://github.com/kazuto1011/r2dm}{Yes} & \\
\cmidrule{1-8}
LiDARDM\cite{zyrianov2025lidardm} & ICRA 25 & multi & SS & map & K,W & \href{https://github.com/vzyrianov/LidarDM}{Yes} & K,W \\
UniScene\cite{li2025uniscene} & CVPR 25 & multi & MM,SS,MV & bev & N & \href{https://github.com/Arlo0o/UniScene-Unified-Occupancy-centric-Driving-Scene-Generation}{Yes} & N \\
Genesis\cite{guo2025genesis} & NeurIPS 25 & multi & MM,SS,MV & layout,object,trajectory & N & \href{https://github.com/xiaomi-research/genesis}{Not yet} &  \\
OpenDWM\cite{ni2025maskgwm} & CVPR 25 & multi & MM,SS,MV & bev & N & \href{https://github.com/SenseTime-FVG/OpenDWM}{Yes} & N \\
LiDARCrafter\cite{liang2026lidarcrafter} & AAAI 26 & multi & SS & text$\rightarrow$layout$\rightarrow$object$\rightarrow$trajectory & N & \href{https://github.com/worldbench/LiDARCrafter}{Yes} &  \\
\cmidrule{1-8}
Our &  & multi & MS & bev,object,semantic & K,N,W & & \\
\bottomrule
\end{tabular}
}
\end{small}
\end{center}
\label{tab:competitors}
\end{table}

==> assets/tables/dm_scene_waymo_side.tex <==
\begin{table}[H]
\begin{center}
\begin{small}
\small
\resizebox{\textwidth}{!}{
    \begin{tabular}{clccccccccccc}
    \toprule
     & \multirow{2}{*}{Method} & \multirow{2}{*}{Input Size} & \multirow{2}{*}{Arch.} & \multirow{2}{*}{Epoch} & \multicolumn{2}{c}{Range} & \multicolumn{2}{c}{Sparse Volume} & \multicolumn{2}{c}{Points} & \multicolumn{2}{c}{BEV} \\
      \cmidrule(l){6-7}
      \cmidrule(l){8-9}
      \cmidrule(l){10-11}
      \cmidrule(l){12-13}
     & & & & & FRID $\downarrow$ & MMD $\downarrow$ & FSVD $\downarrow$ & MMD $\downarrow$ & FPVD $\downarrow$ & MMD $\downarrow$ & JSD $\downarrow$ & MMD $\downarrow$ \\
    \midrule
    \rowcolor{gray!30}
    \multirow{6}{*}{Stacked} &  LiDM-DiT$^{\dagger}$ & 4x52x38 & DiT & 50(37) & 0.457 &   0.0007 & 58.177 & 0.1134 & 11.414 & 0.0187 & 0.1540 & 1.0394 \\
     & LiDM\cite{ran2024towards}$^{\dagger}$\textbf{{\textcolor{blue}{$\ast$}}} & 4x52x40 & UNet & 50(26) & 2.292 & 0.0148 & 17.766 & 0.0262 & 4.6770 & 0.0065 & 0.1934 & 1.0085 \\
     \rowcolor{gray!30}
     & RangeLDM-DiT$^{\dagger}$ & 4x26x76 & DiT & 50(30) & 9.071 & 0.0938 & 150.50 & 0.2305 & 61.476 & 0.0374 & 0.1969 & 1.1575 \\
     \rowcolor{gray!30}
     & RangeLDM-DiT$^{\dagger}$\textbf{{\textcolor{blue}{$\ast$}}} & 4x25x75 & DiT & 50() &  &  & (p) &  &  &  &  &  \\
     & RangeLDM\cite{hu2024rangeldm}$^{\dagger}$\textbf{{\textcolor{blue}{$\ast$}}} & 4x28x76 & UNet & 50(26) & 10.972 & 0.0979 & 279.85 & 0.4299 & 122.38 & 0.1236 & 0.2233 & 1.6353 \\
     & R2DM\cite{nakashima2024lidar} & - & - & - & 216.32 & 2.2839 & 112.98 & 0.1922 & 40.567 & 0.02281 & 0.2754 & 1.9715 \\
    \cmidrule{1-13}
    & LidarDM\cite{zyrianov2025lidardm} &  &  &  &  &  &  &  &  \\
    & Ours & 4x25x75 & DiT &  &  &  &  &  &  &  &  \\
    \bottomrule
    \end{tabular}
}
\end{small}
\end{center}
\caption{\textbf{Scene-level Evaluation of DMs} from different methods on Waymo SIDE LiDAR. \emph{\textbf{Scene}} is composed of multi-sensor LiDAR data. \textcolor{gray}{\textbf{Gray}} color denotes our modified baselines. MMD are reported in 10$^{-4}$ Best metrics are highlighted in \textbf{\textcolor{red}{red}}.}
\label{tab:dm_scene_waymo_side}
\end{table}

==> assets/tables/dm_sensor_waymo_side.tex <==
\begin{table}[H]
\begin{center}
\begin{small}
\small
\resizebox{\textwidth}{!}{
    \begin{tabular}{clcccccccc}
    \toprule
     & Method & Input Size & Arch. & Epoch & FRID $\downarrow$ & FSVD $\downarrow$ & FPVD $\downarrow$ & JSD $\downarrow$ & MMD $\downarrow$ \\
    \midrule
    \rowcolor{gray!30}
    \multirow{5}{*}{Naive} & LiDM-DiT$^{\dagger}$ & 52x38 & DiT  & 50(20) & 2.590 & 40.510 & 6.937 & 0.1268 & 0.4443 \\
     & LiDM\cite{ran2024towards}$^{\dagger}$\textbf{{\textcolor{blue}{$\ast$}}} & 52x40 & UNet & 50(30) & 9.915 & 20.736 & 7.356 & 0.1086 &  4.4572 \\
     \rowcolor{gray!30}
     & RangeLDM-DiT$^{\dagger}$ & 26x76 & DiT & 50(24) & 3.774 & 10.853 & 2.860 & 0.4514 & 0.7447 \\
     \rowcolor{gray!30}
     & RangeLDM-DiT$^{\dagger}$\textbf{{\textcolor{blue}{$\ast$}}} & 25x75 & DiT & 50 & (p) &  &  &  &  \\
     & RangeLDM\cite{hu2024rangeldm}$^{\dagger}$\textbf{{\textcolor{blue}{$\ast$}}} & 28x76 & UNet & 50(30) & 11.926 & 13.579 & 2.617 & 0.1071 & 3.2608 \\
    \cmidrule{1-10}
    \rowcolor{gray!30}
    \multirow{5}{*}{Stacked} & LiDM-DiT$^{\dagger}$ & 4x52x38 & DiT & 50(37) & 0.457 & 36.886 & 2.7274 & 0.1535 & 0.4959 \\
     & LiDM\cite{ran2024towards}$^{\dagger}$\textbf{{\textcolor{blue}{$\ast$}}} & 4x52x40 & UNet & 50(26) & 2.292 & 15.974 & 2.393 & 0.2259 & 3.0496 \\
     \rowcolor{gray!30}
     & RangeLDM-DiT$^{\dagger}$ & 4x26x76 & DiT & 50(30) & 9.071 & 112.56 & 130.46 & 0.1948 & 0.5956 \\
     & RangeLDM-DiT$^{\dagger}$\textbf{{\textcolor{blue}{$\ast$}}} & 4x25x75 & DiT & 50 & (p) &  &  &  &  \\
     & RangeLDM\cite{hu2024rangeldm}$^{\dagger}$\textbf{{\textcolor{blue}{$\ast$}}} & 4x28x76 & UNet & 50(26) & 10.972 & 196.38 & 106.82 & 0.2458 & 2.8490 \\
     & R2DM\cite{nakashima2024lidar} & - & - & - &  &  &  & 0.2635 & 10.2907 \\
    \cmidrule{1-10}
    & LidarDM\cite{zyrianov2025lidardm} &  &  &  &  &  &  \\
    & Ours & 4x25x75 & DiT &  &  &  &  &  &  \\
    \bottomrule
    \end{tabular}
} 
\end{small}
\end{center}
\caption{\textbf{Sensor-level Evaluation of DMs} from different methods on Waymo SIDE LiDAR. Configuration $\dagger$: Densify, Fill Noise, Compression rate $f=64$, Batch Size 16, log transformation, [-1; 1] normalization, etc. \emph{\textbf{Naive}}: each sensor data is treated as an independent sample; \emph{\textbf{Stacked}}: 4 x sensor data of the same scene is stacked together as one sample. \textbf{DiT}: 129.8M params, \textbf{UNet}: 259M params. \textcolor{gray}{\textbf{Gray}} color denotes our modified baselines. MMD are reported in $10^{-4}$}
\label{tab:dm_sensor_waymo_side}
\end{table}


==> assets/tables/dm_video_waymo_side.tex <==
\begin{table}[H]
\begin{center}
\begin{small}
\small
\resizebox{\textwidth}{!}{
    \begin{tabular}{clccccccccccc}
    \toprule
     & \multirow{2}{*}{Method} & \multirow{2}{*}{Input Size} & \multirow{2}{*}{Arch.} & \multirow{2}{*}{Epoch} & \multicolumn{2}{c}{Range} & \multicolumn{2}{c}{Sparse Volume} & \multicolumn{2}{c}{Points} & \multicolumn{2}{c}{BEV} \\
      \cmidrule(l){6-7}
      \cmidrule(l){8-9}
      \cmidrule(l){10-11}
      \cmidrule(l){12-13}
     & & & & & FRID $\downarrow$ & MMD $\downarrow$ & FSVD $\downarrow$ & MMD $\downarrow$ & FPVD $\downarrow$ & MMD $\downarrow$ & JSD $\downarrow$ & MMD $\downarrow$ \\
    \midrule
    \rowcolor{gray!30}
    \multirow{6}{*}{Stacked} &  LiDM-DiT$^{\dagger}$ & 4x52x38 & DiT & 50(37) & 1.873 &  & 58.177 &  & 11.414 &  & 0.1540 & 1.0394 \\
     & LiDM\cite{ran2024towards}$^{\dagger}$\textbf{{\textcolor{blue}{$\ast$}}} & 4x52x40 & UNet & 50(26) & 2.292 &  & 17.766  &  & 4.6770 &  & 0.1934 & 1.0085 \\
     \rowcolor{gray!30}
     & RangeLDM-DiT$^{\dagger}$ & 4x26x76 & DiT & 50(30) & 67.688 &  & 150.50 &  &  61.476 &  & 0.1969 & 1.1575 \\
     \rowcolor{gray!30}
     & RangeLDM-DiT$^{\dagger}$\textbf{{\textcolor{blue}{$\ast$}}} & 4x25x75 & DiT & 50 &  &  & (p) &  &  &  &  &  \\
     & RangeLDM\cite{hu2024rangeldm}$^{\dagger}$\textbf{{\textcolor{blue}{$\ast$}}} & 4x28x76 & UNet & 50(26) & 10.972 &  & 279.85  &  & 122.38 &  & 0.2233 & 1.6353 \\
     & R2DM\cite{nakashima2024lidar} & - & - & - &  &  &  &  &  &  \\
    \cmidrule{1-13}
    & LidarDM\cite{zyrianov2025lidardm} &  &  &  &  &  &  &  &  \\
    & Ours & 4x25x75 & DiT &  &  &  &  &  &  &  &  \\
    \bottomrule
    \end{tabular}
}
\end{small}
\end{center}
\caption{\textbf{Scene-level Evaluation of DMs} from different methods on Waymo SIDE LiDAR. \emph{\textbf{Scene}} is composed of multi-sensor LiDAR data. \textcolor{gray}{\textbf{Gray}} color denotes our modified baselines. MMD are reported in 10$^{-4}$ Best metrics are highlighted in \textbf{\textcolor{red}{red}}.}
\label{tab:dm_scene_waymo_side}
\end{table}

==> assets/tables/image_multi_sensor_waymo.tex <==
\begin{table}[htb!]
\centering
\caption{%
    \textbf{Evaluations of scene-level fidelity for multi-sensor LiDAR generation on Waymo dataset}.
    MMD values are reported in $10^{-4}$ and JSD in $10^{-2}$.
    Lower is better for all metrics.
    TODO:
    Khanh: computes evaluation from Manu's output.
    Carlos: may try to retrain opendwm.
}%
\label{tab:video_multi_sensor_waymo_image_based}
\small
\setlength{\tabcolsep}{4pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{lllrrrrrr}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Venue} &
\multirow{2}{*}{Who is work. on} &
\multicolumn{2}{c}{Range} &
\multicolumn{2}{c}{Points} &
\multicolumn{2}{c}{BEV} \\
\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
& & & FRD$\downarrow$ & MMD$\downarrow$ & FPD$\downarrow$ & MMD$\downarrow$ & JSD$\downarrow$ & MMD$\downarrow$ \\
\midrule
\multicolumn{8}{l}{\textbf{Voxel}}\\
UniScene\cite{li2025uniscene}      & CVPR'25 &  & --     & --    &  &  &  &  \\
OpenDWM                            & CVPR'25 &  & --     & --    &  &  &  &  \\
OpenDWM-DiT                        & CVPR'25 &  & --     & --    &  &  &  &  \\
\midrule
\multicolumn{8}{l}{\textbf{Range}}\\
%LiDARGen\cite{zyrianov2022learning}                                 & ECCV'22 & Steve &  \multicolumn{6}{c}{Not included}  \\
LiDM\cite{ran2024towards}  & CVPR'24 &  Khanito  & 2.29 & 148.83 & 4.67 & 65.76 & 19.34 & 1.00 \\
RangeLDM\cite{hu2024rangeldm} & ECCV'24 &  Khanito & 10.97 & 979.33 & 122.38 & 1236.59 & 22.33 & 1.63 \\
R2DM\cite{nakashima2024lidar}             & ICRA'24 & Carlitos & 216.32 & 2283.90 & 40.56 & 228.04 & 27.54 & 1.97 \\
\cellcolor[HTML]{cfe2f3}{LidarDM\cite{zyrianov2025lidardm}} & ICRA'25 & Khanito &  &  &  &  &  &  \\
\multicolumn{8}{l}{\textbf{Range-Temporal}}\\
\cellcolor[HTML]{cfe2f3}{LiDM\cite{ran2024towards}(t=5)}  &  &  Khanito &  &  &  &  &  \\
\cellcolor[HTML]{cfe2f3}{RangeLDM\cite{hu2024rangeldm}(t=5)} &  & Khanito &  &  &  &  &  &  \\
%LiDARCrafter\cite{liang2025lidarcrafter}  & AAAI'26 &  &  &  &  &  &  \\
\midrule
\rowcolor[HTML]{F5D0CB}
\lname            & Evaluation & Khanh\&Manu & ---    & ---   & ---    &   --- &   --- &   --- \\
\bottomrule
\end{tabular}
}
\end{table}
   

==> assets/tables/waymo_stats_anno.tex <==
\begin{table*}[t]
    \centering
    \begin{minipage}{0.3\textwidth}
        \centering
            \begin{tabular}{c}
                \begin{tabular}{lccc}
                    \toprule
                     & TrainVal & Test\\
                    \midrule
                    \texttt{Vehicle} & 941.6K & 227K \\
                    \texttt{Pedestrian} & 499.1K & 121.4K \\
                    \texttt{Cyclist} & 11.8K & 3.4K \\
                    \midrule
                    Total & 1451.6K & 352K \\
                    \bottomrule
                \end{tabular}
                \label{tab:waymo_3d_anno}
            \end{tabular}
        \caption{\textbf{Statistics} on annotations.}
        \label{tab:waymo_anno_stats}
    \end{minipage}
    \hfill
    \begin{minipage}{0.33\textwidth}
        \centering
            \begin{tabular}{r}
                \begin{tabular}{cccc}
                    \toprule
                     & Train & Val & Test\\
                    \midrule
                     Scenes & 798 & 202 & 150 \\
                     Frames & 158K & 40K & 30K \\
                     Clips & 21K & 5K & 5K \\
                    \bottomrule
                \end{tabular}
            \end{tabular}
    \caption{\textbf{Size} of the data splits.}
    \label{tab:waymo_split}
    \end{minipage}
    \begin{minipage}{0.30\textwidth}
        \centering
        \includegraphics[width=\linewidth]{assets/graphics/waymo_side_frame_count.png}
    \caption{\textbf{Per-frame} Annotations.}%
    \label{fig:waymo_per_frame}
    \end{minipage}
\end{table*}

